Continual Learning of Natural Language Processing Tasks: A Survey

Continual learning (CL) is a learning paradigm that emulates the human capability of learning and accumulating knowledge continually without forgetting the previously learned knowledge and also transferring the learned knowledge to help learn new tasks better. This survey presents a comprehensive review and analysis of the recent progress of CL in NLP, which has significant differences from CL in computer vision and machine learning. It covers (1) all CL settings with a taxonomy of existing techniques; (2) catastrophic forgetting (CF) prevention, (3) knowledge transfer (KT), which is particularly important for NLP tasks; and (4) some theory and the hidden challenge of inter-task class separation (ICS). (1), (3) and (4) have not been included in the existing survey. Finally, a list of future directions is discussed.

==> tables/settings.tex <==

\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|ccccc}
\specialrule{.2em}{.1em}{.1em}
 &  & \textbf{Conventional Property} & \textbf{Task Type} & \textbf{Property} & \textbf{Tasks} & \textbf{Desiderata} \\
  \specialrule{.1em}{.05em}{.05em} 
\multirow{9}{*}{\textbf{Settings}} &
\multirow{6}{*}{Task-IL} & \multirow{6}{*}{} &  Conventional & each task has sufficient data & end-task \\  
\cline{4-6}
&  &  & Few-shot & each task is few-shot learning task & end-task \\  
\cline{4-6}
 &  &  & Cpre & {\begin{tabular}[c]{@{}c@{}} evaluated by end-task \\ task-ID only provided in pre-training\end{tabular}} & domain corpus \\  
 \cline{4-6}
 &  &  & Cpos & {\begin{tabular}[c]{@{}c@{}} no access to pre-training data\\ evaluated by end-task \\ task-ID only  provided in pre-training \end{tabular}} & domain corpus \\ 
\cline{2-7}
& Domain-IL & &  & end-task &  \multirow{6}{*}{{\begin{tabular}[c]{@{}c@{}}CF prevention \\  directional KT\end{tabular}}} \\
\cline{2-7}
 & \multirow{2}{*}{Class-IL} & & Conventional & each task has sufficient data  & end-task & {\begin{tabular}[c]{@{}c@{}} CF prevention \\  bi-directional KT \\ task-ID prediction \end{tabular}}\\
 \cline{4-6}
  &  &  & Few-shot & each task is few-shot learning task & end-task \\  
 \cline{2-7}
 & \multirow{4}{*}{Temporal-IL} & \multirow{4}{*}{{\begin{tabular}[c]{@{}c@{}}  Similar to Task-IL but $t$ is continuous\\ $D_t$ could sudden or gradual changes \\ to $D_{t+\tau}$ at any moment \end{tabular}} } & Cpre & {\begin{tabular}[c]{@{}c@{}} evaluated by end-task \\ time given in pre-training and end-task \end{tabular}}  & temporal corpus & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}CF Prevention \\  bi-directional KT\end{tabular}} \\
  \cline{4-6}
  &  &  & Cpos & {\begin{tabular}[c]{@{}c@{}} no access to pre-training data\\ evaluated by end-task \\ time given in post-training and end-task \end{tabular}} & temporal corpus \\
  \hline
\multirow{3}{*}{\textbf{Modes}} & \multirow{2}{*}{Online} & \multirow{2}{*}{train only one single epoch} & Hard Boundary & clear task split without task-ID & \multicolumn{2}{c}{\multirow{3}{*}{depends on settings}} \\ \cline{4-5}
 &  &  & Blurry Boundary & task data is mixed with other tasks\\ \cline{2-5}
 & Offline & train any \#epochs &  Hard Boundary &  clear task split
 \\ \specialrule{.1em}{.05em}{.05em}
\end{tabular}
}
\caption{\zixuan{need re-org}Different Settings and modes for continual learning.
We can can see the conventional task-IL takes task-ID as input in both training and testing while class-IL takes task-ID as input in training but no task-ID avaialable in testing. \bing{DIL should be included but describe it as a special case of TIL.}
}
 \vspace{-4mm}
\label{tab:set_mode}
\end{table*}


